On the Evaluation of Large Language Models in Unit Test Generation

Unit testing is an essential activity in software development for verifying the correctness of software components. However, manually writing unit tests is challenging and time-consuming. The emergence of Large Language Models (LLMs) offers a new direction for automating unit test generation. Existing research primarily focuses on closed-source LLMs (e.g., ChatGPT and CodeX) with fixed prompting strategies, leaving the capabilities of advanced open-source LLMs with various prompting settings unexplored. Particularly, open-source LLMs offer advantages in data privacy protection and have demonstrated superior performance in some tasks. Moreover, effective prompting is crucial for maximizing LLMs' capabilities. In this paper, we conduct the first empirical study to fill this gap, based on 17 Java projects, five widely-used open-source LLMs with different structures and parameter sizes, and comprehensive evaluation metrics. Our findings highlight the significant influence of various prompt factors, show the performance of open-source LLMs compared to the commercial GPT-4 and the traditional Evosuite, and identify limitations in LLM-based unit test generation. We then derive a series of implications from our study to guide future research and practical use of LLM-based unit test generation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Sections/Introduction.tex <==
\section{Introduction}
In the current landscape of Artificial Intelligence (AI) research, Large-scale Language Models (LLMs) have gained massive attention and are transforming the way we approach and comprehend language tasks. These models, characterized by their immense scale and capacity to learn, have become synonymous with breakthroughs in many domains. For example, in Code-Related tasks such as code comprehension and code generation, many LLMs have shown unprecedented ability, revolutionizing how developers approach coding challenges. Furthermore, programming assistants such as Copilot have already started helping developers finish their tasks and have shown remarkable ability in coding.

Although LLMs have shown enormous effectiveness in general code generation and have been widely studied on the HumanEval benchmark, in the realm of specific software engineering tasks such as Unit Test Generation, there is a lack of concrete empirical study.
First, existing LLM-based unit test generation research mainly focus on ChatGPT~\cite{chatunitest,chattester}, which is by far the most powerful model but is not representative since it is close-source and the details of its training process are blind to users or researchers.
Second, there is a lack of high-quality open-source benchmarks such as HumanEval, and an existing dataset such as method2tests is not quite suitable for evaluating LLM due to its lack of sufficient context information. Furthermore, the existing study~\cite{evalplus} has shown that HumanEval-based performance does not really reveal its true ability and that three test cases are not enough for a comprehensive comparison. Therefore, a high-quality benchmark is of great importance for the progress of research. 

Another serious challenge in adopting LLMs is its significant resource requirements, such as time and computing power. For example, training CodeLlama with 7 billion parameters in 16-bit precision will need more than 50 GB of GPU memory, and with limited computing resources, the time cost of training will grow explosively. This huge cost has a significant impact on both academic research and the practical use of LLMs. To mitigate this challenge, researchers have been focusing on prompt engineering and have proposed several techniques based on zero-shot or few-shot learning. However, existing research~\cite{cedar} has shown that the selection of examples has a significant impact on the effectiveness of few-shot learning.
Unlike prompt engineering, previous deep-learning-based techniques usually adopted supervised fine-tuning to improve the effectiveness of pre-trained language models in specific programming tasks such as test case generation. However, such a high resource cost creates a barrier to entry for many researchers, limiting access to cutting-edge technology. 

Unit testing is one of the most significant parts of software testing and plays a fundamental guarantee that the implementation of the functionality is as expected. Unit test generation has been studied for decades. Traditional unit test generation techniques, such as Evosuite~\cite{evosuite} and Randoop~\cite{randoop}, adopt static analysis techniques to analyze input and output of the program and synthesize unit test cases according to the results. Recently, ChatTester~\cite{chattester}, which is the state-of-the-art unit test generation technique based on ChatGPT, has shown that compared to traditional techniques, although the test cases generated by ChatGPT suffer from compilation and execution errors, they achieved comparable coverage score to manual tests and are closer to the latter compared to those generated by traditional ones. Furthermore, the authors have found that the interviewees are willing to directly adopt the ChatGPT-generated tests. Such results show that LLMs have real potential to be a test agent and significantly accelerate the automation of software testing. 
However, ChatGPT is one of a kind. For example, it accepts inputs of up to 128,000 tokens, while the majority of open-source LLMs are around 16,000. Longer inputs can include more context information and could help LLMs understand the instruction. For example, ChatUniTest~\cite{chatunitest} proposed an Adaptive Focal Context Generation algorithm, so that the prompt can involve as many contextual features as possible within the maximum prompt length of ChatGPT. However, on the bad side, long inputs will lead to a substantial increase in the demand for resources and significantly hinder the practical use of LLMs, including ChatGPT. Consequently, a more comprehensive study on the practical use of LLMs in generating unit tests is needed.

Therefore, in this study, we conducted the first empirical study on open-source state-of-the-art LLMs to investigate their effectiveness in unit test generation. 
Here, we tend to addressed four research question to comprehensively investigating the performance of LLMs in unit test generation:

\begin{itemize}
    \item RQ1: How do state-of-the-art LLMs perform in unit test generation?
    \item RQ2: How does the selection of context features affect the effectiveness of LLMs in terms of unit test generation?
    \item RQ3: Will supervised fine-tuning (SFT) based on the prompts targeted at unit test generation help with the performance?
    \item RQ4: How good do the unit tests generated by LLMs in terms of finding bugs?
\end{itemize}


First, we selected five state-of-the-art LLMs with different scales and HumanEval scores from the open-source model hosting website Huggingface~\cite{huggingface}, namely CodeLlama-7b-Instruct, CodeLlama-13b-Instruct, deepseek-coder-6.7b-instruct, deepseek-coder-33b-instruct~\cite{deepseek-coder}, and Phind-34B-CodeLlama-v2. They are both fine-tuned by code-related tasks such as code generation and have shown promising results based on the HumanEval benchmark. 
Second, to evaluate their performance on unit test generation, following the experimental settings of previous research~\cite{a3test, chatunitest}, we used the Defects4J 2.0 benchmark for evaluation. Defects4j has been widely used to evaluate the performance of bug detection~\cite{?} and bug fixing techniques~\cite{?}. It contains 835 real bugs from 17 GitHub repositories, and each bug has a buggy version and a fixed version along with multiple unit test cases in each version. The unit test that fails in the buggy version but passes in the fixed version is called \textit{\textbf{bug-triggering test}}, and the difference between the execution results means that the test case successfully finds a bug. Since the objective of unit testing is to find bugs in the method under test, the ability to generate bug-triggering tests is also a crucial metric for unit test generation techniques. Therefore, in our study, we evaluated the performance of LLMs in terms of generating unit tests by three metrics: the compile rate, the coverage score (including both line coverage and branch coverage) and the number of bugs found.

Our results show that \yl{larger scale LLMs indeed perform better than smaller ones, but the ability of LLMs in code generation does not necessarily equal to that in unit test generation, since higher HumanEval score does not lead to higher compile rate and coverage score. Furthermore, we found that LLMs are sensitive to contextual features. For example, a lack of critical information, such as parameters, could lead to a drastic decrease in the compile rate. Last but not least, we fine-tuned some of the studied LLMs to the best of our ability and found that smaller models after supervised fine-tuning could be largely improved since the output is more fit to the unit test generation, while the improvement of fine-tuning larger models over using pre-trained ones is smaller. To comprehensively understand the gap between the practical use of LLMs and the claimed performance, we further conducted a case study to show some of the representative errors while compiling the unit tests generated by LLMs. In summary, LLMs can actually generate codes that are semantically right but lack constraint, as they often generate a token that appears semantically correct, but cannot be found.}











==> Sections/Study_Design_RQs.tex <==
\subsection{Research Questions}
\yl{move the following introduction of research questions to study design.}


% Our experimental results indicate that the effectiveness of open-source LLMs varies slightly with different styles of task descriptions. However, as the capabilities of the models improve, their robustness to variations in task descriptions also increases. 
% Additionally, we observed that certain types of context feature, such as other methods (as opposed to the focal method) in the class under test, can introduce noise. This finding underscores the importance of carefully selecting and structuring the code context features provided to open-source LLMs to optimize their performance and minimize the introduction of irrelevant or misleading data. One possible solution is to incorporate traditional static program analysis techniques, such as call graph or dependency graph, in filtering context features.



% Our experimental results indicate that the effectiveness of open-source LLMs in generating unit tests still lags behind GPT-4 and Evosuite, primarily due to hallucination issues. These issues lead to numerous compilation errors that significantly affect their effectiveness. However, integrating traditional software analysis techniques to reduce the vast search space of LLMs could mitigate hallucination issues and substantially improve the effectiveness of open-source LLMs in generating high-quality unit tests.

% Our experimental results indicate that the contribution of in-context learning techniques to the effectiveness of LLMs in unit test generation is minimal. Furthermore, we identified several challenges in adapting in-context leaning techniques in open-source LLMs. Based on these findings, we recommend that when employing in-context learning techniques, the focus should shift from the specifics of code implementation to the functionality of the function under test and the testing scenarios. For instance, providing information about testing scenarios within the in-context learning framework could guide the model to generate test cases that are specifically tailored to those scenarios. This approach ensures that the test cases are more aligned with the real-world applications they are intended to validate, potentially enhancing the effectiveness of the generated test cases.


Last but not least, since the goal of unit testing is to identify defects within the production code, the defect detection capability of unit tests is a critical metric. 
Therefore, we also conducted experiments on the defect detection capabilities of the unit tests generated by open-source LLMs. Specifically, we adhered to the experimental settings of previous studies~\cite{d4jtestset} and executed unit tests on both buggy and fixed versions of the production code. A unit test that passes on the fixed version but fails on the buggy version indicates a detected defect. We compared the number of detected defects of unit tests generated by different open-source LLMs to answer the following Research Question:



% Our experimental results indicate that the defect detection capabilities of unit tests generated by open-source LLMs currently do not meet the testing requirements. Building on this, we further analyzed the strengths and weaknesses of them. 
% For relatively simple methods with clear functionality, LLMs can understand their purpose and various application scenarios well, making it easier to detect defects. However, for more complex functions with intricate branches, LLMs struggle to comprehend their functionality and application scenarios, making defect detection more difficult.
% The analysis showed that open-source LLMs have a relatively good capability to detect defects in methods with clear functionalities (e.g., Matrix Multiplication). However, their ability to detect defects in methods with complex branch conditions is weaker.
% These results emphasize that there should be a focused consideration on the target functionality of the focal method. In addition, it is crucial to cover as many application scenarios as possible. This approach will help in enhancing the models' ability to detect subtle and complex defects that might occur under varied operational conditions.

==> data/name.tex <==
import numpy as np
from scipy.stats import mannwhitneyu, rankdata

def calculate_wilcoxon_rank_sum(x, y):
    # 计算Wilcoxon rank sum的p值
    stat, p_value = mannwhitneyu(x, y, alternative='two-sided')
    
    # 计算rank-biserial correlation效应量
    n1, n2 = len(x), len(y)
    rank_x = np.mean(rankdata(np.concatenate([x, y]))[:n1])
    rank_y = np.mean(rankdata(np.concatenate([x, y]))[n1:])
    rbc = (rank_x - rank_y) / (n1 + n2)
    
    return p_value, rbc

# 示例数据
data1 = np.random.normal(0, 1, 100)  # 第一组数据
data2 = np.random.normal(0.5, 1, 100)  # 第二组数据

# 计算
p_value, rbc = calculate_wilcoxon_rank_sum(data1, data2)
print("Wilcoxon rank sum test p-value:", p_value)
print("Rank-biserial correlation:", rbc)


==> listings/autocot_example.tex <==
\begin{lstlisting}[language=Markdown, caption=Illustrating example of AutoCoT postfix., label=lst:AutoCoT_Postfix]
    Your task is to write unit tests in Java 1.7 and Junit 4 with maximizing both branch and line coverage. 
    Let's first understand the problem and devise a plan to solve the problem. 
    Then, let's carry out the plan and solve the problem **step by step**.
\end{lstlisting}

==> listings/cot_example.tex <==
\begin{lstlisting}[language=Markdown, caption={Illustrating example of Thought About the Functionality, Branches and Input-Output Expections}, label=lst:CoT_Example]
This Java function, `looksLikeOption`, checks if a given string (`trigger`) resembles an option based on certain prefixes and conditions:

1. **Functionality:** The function iterates over a collection of `prefixes`. If `trigger` starts with any of these prefixes and either `getCurrentOption().canProcess(this, trigger)` returns `true` or `getCurrentOption().findOption(trigger)` is not `null`, the function returns `true`. Otherwise, it returns `false`.
2. **Branches:**
    - **Branch 1:** `checkForOption != null` - This is a reentrant call, and the function returns the negation of the comparison between `checkForOption` and `trigger`.
    - **Branch 2:** `trigger.startsWith(prefix)` - If `trigger` starts with a prefix.
    - **Branch 3:** `getCurrentOption().canProcess(this, trigger)` or `getCurrentOption().findOption(trigger) != null` - If the current option can process the trigger or finds an option for the trigger.
3. **Input-Output Expectations:**
    - **Branch 1:** Input: `trigger = "option1"`, `checkForOption = "option2"`; Output: `true`
    - **Branch 2:** Input: `trigger = "opt1"`, `prefixes = ["opt", "cmd"]`; Output: Depends on the result of `getCurrentOption()` methods.
    - **Branch 3:** Input: `trigger = "opt1"`, `getCurrentOption().canProcess(this, "opt1") = true`; Output: `true`

The actual output for Branch 2 and Branch 3 would depend on the implementation of `getCurrentOption()` and its methods.

\end{lstlisting}

==> listings/cot_results.tex <==
% \begin{figure}[h]
%     \centering
%     \begin{minipage}{0.47\textwidth}
%         \begin{lstlisting}[language=java, caption=A Focal Method in a Good Case, label=lst:good_input, basicstyle=\fontsize{7}{9}\selectfont]
% public EqualsBuilder append(long[] lhs, long[] rhs) {
%     if (isEquals == false) { return this; }
%     if (lhs == rhs) { return this; }
%     if (lhs == null || rhs == null) {
%         ...
%         return this;
%     }
%     if (lhs.length != rhs.length) {
%         ...
%         return this;
%     }
%     for (int i = 0; i < lhs.length && isEquals; ++i) { ... }
%     return this;
% }
%         \end{lstlisting}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.47\textwidth}
%         \begin{lstlisting}[language=java, caption=A Focal Method in a Bad Case , label=lst:bad_input, basicstyle=\fontsize{7}{9}\selectfont]
% public static Number createNumber(String str) throws NumberFormatException {
%     if (str == null) {
%         return null;
%     }
%     if (StringUtils.isBlank(str)) {
%         throw new NumberFormatException("A blank string is not a valid number");
%     }
%     ...
%     ...
%     ...
%     ...
%     ...
%     ...
% }
%         \end{lstlisting}
%     \end{minipage}
%     % \caption{Illustrating Examples of Results}
%     % \label{fig:cot_results}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{minipage}{0.47\textwidth}
%         \begin{lstlisting}[language=Markdown, caption=A Result in a Good Case, label=lst:good_output, basicstyle=\fontsize{7}{9}\selectfont]
% ...
% 1. Functionality: ...
% 2. Branches:
%    - Branch 1: isEquals == false 
%    - Branch 2: lhs == rhs 
%    - Branch 3: lhs == null || rhs == null 
%    - Branch 4: lhs.length != rhs.length 
%    - Branch 5: lhs.length == rhs.length 
% 3. Input-Output Expectations:
%    - Branch 1: Input: lhs = [1, 2, 3], rhs = [1, 2, 3], isEquals = false; 
%    - Branch 2: Input: lhs = [1, 2, 3], rhs = [1, 2, 3], isEquals = true; 
%    - Branch 3: Input: lhs = null, rhs = [1, 2, 3]; 
%    - Branch 4: Input: lhs = [1, 2, 3], rhs = null; 
%    - Branch 5: Input: lhs = [1, 2, 3], rhs = [4, 5, 6]; 
% In summary, ...
%         \end{lstlisting}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.47\textwidth}
%         \begin{lstlisting}[language=Markdown, caption=A Result in a Bad Case , label=lst:bad_output, basicstyle=\fontsize{7}{9}\selectfont]
% ...
% The method has multiple branches that handle different cases, including:

% 1. Checking if the input string is null or blank, and throwing an exception if it is.
% 2. ...

% The input-output expectations for each branch are as follows:

% 1. Input: null, Output: throws NumberFormatException.
% 2. ...

% ...
%         \end{lstlisting}
%     \end{minipage}
%     % \caption{Illustrating Examples of Results}
%     % \label{fig:cot_results}
% \end{figure}





\begin{figure}[ht]
  \begin{subfigure}{0.47\linewidth}
    \begin{minipage}[t]{\linewidth}
      \begin{lstlisting}[language=java, label=lst:good_input, basicstyle=\fontsize{7}{9}\ttfamily]
public EqualsBuilder append(long[] lhs, long[] rhs) {
    if (isEquals == false) { return this; }
    if (lhs == rhs) { return this; }
    if (lhs == null || rhs == null) { ... }
    if (lhs.length != rhs.length) { ... }
    for (int i = 0; i < lhs.length && isEquals; ++i) { ... }
    return this;
}
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[b]{\linewidth}
      \begin{lstlisting}[language=Markdown, label=lst:good_output, basicstyle=\fontsize{7}{9}\selectfont]
...
This Java method, append, is part of the EqualsBuilder class and is used to compare two long arrays for equality.
1. Functionality: 
   - It first checks if ...
   ...
2. Branches:
   - Branch 1: isEquals == false 
   - Branch 2: lhs == rhs 
   - Branch 3: lhs == null || rhs == null 
   - Branch 4: lhs.length != rhs.length 
   - Branch 5: lhs.length == rhs.length 
3. Input-Output Expectations:
   - Branch 1: Input: lhs = [1, 2, 3], rhs = [1, 2, 3], Output...; 
   - Branch 2: Input: lhs = [1, 2, 3], rhs = [1, 2, 3], Output...;
   - Branch 3: Input: lhs = null, rhs = [1, 2, 3]; Output...;
   - Branch 4: Input: lhs = [1, 2, 3], rhs = [1, 2, 3, 4]; Output...;
   - Branch 5: Input: lhs = [1, 2, 3], rhs = [4, 5, 6]; Output...;

      \end{lstlisting}
    \end{minipage}
    \caption{Good Case}
    % \label{fig:leftgroup}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.47\linewidth}
    \begin{minipage}[t]{\linewidth}
      \begin{lstlisting}[language=java, label=lst:bad_input, basicstyle=\fontsize{7}{9}\ttfamily]
public static Number createNumber(String str) throws NumberFormatException {
    if (str == null) {
        return null;
    }
    if (StringUtils.isBlank(str)) {
        throw new NumberFormatException("A blank string is not a valid number");
    }
    ...
    ...
    ...
    ...
    ...
    ...
}
      \end{lstlisting}
    \end{minipage}
    \begin{minipage}[b]{\linewidth}
      \begin{lstlisting}[language=Markdown, label=lst:bad_output, basicstyle=\fontsize{7}{9}\selectfont]
...
The method has multiple branches that handle different cases, including:

1. Checking if the input string is null or blank, and throwing an exception if it is.
2. ...

The input-output expectations for each branch are as follows:

1. Input: null, Output: throws NumberFormatException.
2. ...

...

      \end{lstlisting}
    \end{minipage}
    \caption{Bad Case}
    % \label{fig:rightgroup}
  \end{subfigure}
  \caption{Illustrating examples of using Chain-of-Thought technique in unit test generation.}
  \label{fig:cot_results}
\end{figure}


==> listings/prompt_example.tex <==
\begin{lstlisting}[language=Markdown, caption=Illustrating example of Instruction Prompt from PD-34B, label=lst:instruction_example]
### System Prompt
You are an intelligent programming assistant.

### User Message
Your task is to write unit tests for ...

### Assistant
Sure! Here are some unit tests...
\end{lstlisting}

==> listings/prompt_strategy_examples.tex <==

% \lstset{
%     language=Markdown,
%     basicstyle=\ttfamily,
%     keywordstyle=\color{blue},
%     commentstyle=\color{gray},
%     stringstyle=\color{red},
%     showstringspaces=false
% }
\begin{figure}[h]
    \centering
    \begin{minipage}{0.45\textwidth}
        \begin{lstlisting}[language=Markdown, caption=Natural Language Style, label=lst:natural-like-strategy]
This is the method you are going to test:
```
{ Focal Method }
```

There are { #Parameter } parameters in the method, namely { Parameter Names }.

Other code context features described in natural language
        \end{lstlisting}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \begin{lstlisting}[language=Markdown, caption=Code Language Style, label=lst:comment-like-strategy]
```
// This is the method you are going to test:
{ Focal Method }

// The parameters of the method:
{ Parameter Names }

// Other code context features decribed in code comments
```
        \end{lstlisting}
    \end{minipage}
    % \caption{Illustrating Examples of Different Prompting Strategies}
    % \label{fig:strategy_example}
\end{figure}

==> listings/rag_example.tex <==
\begin{lstlisting}[language=Java, caption=Illustrating example of retrieved similar focal method and corresponding unit test(s), label=lst:RAG_Example, basicstyle=\ttfamily\footnotesize]
Here is an example of a similar focal method and its unit test(s):
```
// The following code is an example focal method.
public int hashCode() {
    if (getLabel() != null) {
        return getLabel().hashCode();
    }
    else {
        return 0;
    }
}
// The following code is the unit test(s) for the example method.
public void testHashCode() {
    DateAxis a1 = new DateAxis("Test");
    DateAxis a2 = new DateAxis("Test");
    assertTrue(a1.equals(a2));
    int h1 = a1.hashCode();
    int h2 = a2.hashCode();
    assertEquals(h1, h2);
}
...
```
\end{lstlisting}

==> listings/unresolved_symbol_and_no_suitable_method.tex <==
\begin{figure}[ht]
\begin{lstlisting}[language=Java, caption=Illustrating example of Unresolved Symbol and No Suitable Method, label=lst:example_1, basicstyle=\ttfamily\footnotesize]
@Test
public void testLinearCombination7() {
    double a1 = 1.0;
    // ...
    double b3 = 6.0;
    
    // Error 1: No Suitable Method linearCombination found.
    // MathArrays.linearCombination only accept 6 parameters, but got 9
    
    // Error 2: Unresolved Symbols: a4 - b9
    double result = MathArrays.linearCombination(a1, b1, a2, b2, a3, b3, 
    a4, b4, a5, b5, a6, b6, a7, b7, a8, b8, a9, b9);
    // ...
}
\end{lstlisting}
\end{figure}

==> tables/RQ1_Prompt_Decision.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The Recommended Prompt Design for studied Open-source LLMs}
\label{tab:prompt_decision}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
                  & CL-7B     & CL-13B    & PD-34B    & DC-7B & DC-33B \\ \midrule
Description Style & Natural   & Natural   & Code      & Code  & Code   \\
Code Features     & w/o $FC_m$ & w/o $FC_m$ & w/o $FC_m$ & Full  & Full   \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/RQ1_compile_error.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The Impact Scope (\%) of 7 Most Frequent Compilation Errors.}
\label{tab:rq1_compilation_errors}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Compilation Error} & \textbf{CL-7B} & \textbf{CL-13B} & \textbf{PD-34B} & \textbf{DC-7B} & \textbf{DC-33B} & \textbf{GPT-4} \\ \midrule
Unresolved Symbol & {35.75} & {32.45} & {19.39} & {20.34} & {20.98} & {21.37} \\
No Suitable Method            & 16.89 & 15.04  & 7.78   & 9.51  & 8.44   & 9.50  \\
Abstract Type Instantiation & 9.37  & 12.53  & 5.01   & 7.27  & 7.39   & 5.15  \\
Accessibility Issue                  & 6.07  & 8.05   & 5.67   & 7.00  & 8.84   & 7.65  \\
Ambiguous References                 & 6.20  & 4.62   & 2.90   & 4.89  & 6.20   & 5.01  \\
Incompatible Types                   & 5.41  & 4.62   & 2.37   & 2.25  & 2.11   & 2.64  \\
Incompatible Constructor    & 6.33  & 4.62   & 1.32   & 1.19  & 1.58   & 1.06  \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/RQ3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\small
\caption{Effectiveness comparison of three studied models and their supervised fine-tuned versions.}
\label{tab:rq3}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{crrrrrr}
    \toprule
    \multirow{2}[2]{*}{\textbf{Metrics}} & \multicolumn{2}{c}{DC-7B} & \multicolumn{2}{c}{CL-7B} & \multicolumn{2}{c}{CL-13B} \\
          & \multicolumn{1}{c}{w/o SFT} & \multicolumn{1}{c}{SFT} & \multicolumn{1}{c}{w/o SFT} & \multicolumn{1}{c}{SFT} & \multicolumn{1}{c}{w/o SFT} & \multicolumn{1}{c}{SFT} \\
    \midrule
    \% Compile & 69.00 & 38.33 & 39.67 & 39.91 & 46.83 & 34.98 \\
    Line Cov. & 39.56 & 40.14 & 41.11 &  37.08 & 32.79 & 34.68 \\
    Branch Cov. & 28.65 & 30.68  & 32.45 & 27.44 & 24.46 & 21.46 \\
    \bottomrule
    \end{tabular}%
}
\end{table}

==> tables/RQ3_compile_rate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\small
\caption{Comparison of Compilation Success Rate Over Different In-Context Learning Techniques\wwj{done}.}
\label{tab:rq3_compile_rate}
\begin{tabular}{@{}l|rrrrr@{}}
% \hline
\toprule
\multicolumn{1}{c|}{\textbf{Model}}    & \textbf{CL-7B}          & \textbf{CL-13B}         & \textbf{PD-34B}         & \textbf{DC-7B}          & \textbf{DC-33B}        \\ 
\midrule 
Base      & 38.17            & 35.52 & 49.07           & 49.22 & 45.65          

% \\
% + CoT     
% & \textcolor{red}{\ul{-5.32}}
% & \textcolor{blue}{\ul{+9.58}}
% & \textcolor{blue}{+3.81}
% & \textcolor{red}{\ul{-5.42}}
% & \textcolor{red}{-1.27}

% % & 40.59          & 42.22          & 49.93          & 38.37          & 43.08          
% % & -4.95
% \\
% % + AutoCoT 
% % % & 33.38          & 37.23          & 53.82          & 43.51          & 44.51          
% % & \textcolor{red}{-4.57}
% % & \textcolor{red}{-13.41}
% % & \textcolor{red}{-1.67}
% % & \textcolor{red}{-5.71}
% % & \textcolor{red}{-1.14}


% % \\
% + RAG     
% % & \textbf{41.16} & 46.79          & \textbf{56.63} & 47.22          & \textbf{46.08} 
% & \textcolor{red}{-2.28}
% & \textcolor{red}{-0.84}
% & \textcolor{red}{\ul{-7.14}}
% & \textcolor{red}{\ul{-5.47}}
% & \textcolor{red}{-1.90}

% \\ \hline


\\
+ CoT     
& {\textbf{-5.32}}
& {\textbf{+9.58}}
& {+3.81}
& {\textbf{-5.42}}
& {-1.27}

\\


% \\
+ RAG     
& {-2.28}
& {-0.84}
& {\textbf{-7.14}}
& {\textbf{-5.47}}
& {-1.90}

\\ \bottomrule

\end{tabular}
\end{table}

==> tables/data_leakage.tex <==

\begin{table}[t]
\centering
\small
\caption{Proportion of test cases that do not invoke the target function}
\label{tab:data_leakage}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
\multirow{2}{*}{} &
  \multicolumn{2}{c}{{\ul CL}} &
  \multicolumn{1}{c}{{\ul PD}} &
  \multicolumn{2}{c}{{\ul DC}} 
  % \multicolumn{1}{c}{\multirow{2}{*}{{\ul GPT-4}}} 
  \\
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{7B} &
  \multicolumn{1}{c}{13B} &
  \multicolumn{1}{c}{34B} &
  \multicolumn{1}{c}{7B} &
  \multicolumn{1}{c}{33B} 
    
  % \multicolumn{1}{c}{}
  \\ 
  \midrule
Percentage & 0.29 & 0.42 & 0.47 & 0.41  & 0.58   \\
Total & 14,528 & 11,599  & 5,879& 4,948  & 9,140    \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Number of passed unit tests of studied LLMs on Defects4J benchmark.}
\begin{tabular}{@{}crrr@{}}
\toprule
Model & \multicolumn{1}{c}{\# Passed UT} & \multicolumn{1}{c}{\# Total Generated} & \multicolumn{1}{c}{Pass Rate (\%)} \\ \midrule
CL-7B  & 4,458 & 10,806 & 41.25 \\
CL-13B & 3,209 & 8,757  & 36.64 \\
PD-34B & 2,155 & 4,871  & 44.24 \\ \midrule
DC-7B  & 3,785 & 5,765  & 65.65 \\
DC-33B & 3,409 & 8,105  & 42.06 \\ \bottomrule
\end{tabular}
\end{table}


==> tables/defects4j_statistics.tex <==
% \begin{table*}[t]
% \caption{Statistics of the bugs and focal methods in our study.}
% \label{tab:defects4j}
% \centering
% \small
% \scalebox{0.6}{
% \begin{tabular}{@{}lrrrrrrrrrrrrrrrrrr@{}}
% \toprule
% Project &
%   \multicolumn{1}{c}{\textbf{Chart}} &
%   \multicolumn{1}{c}{\textbf{Cli}} &
%   \multicolumn{1}{c}{\textbf{Closure}} &
%   \multicolumn{1}{c}{\textbf{Codec}} &
%   \multicolumn{1}{c}{\textbf{Collections}} &
%   \multicolumn{1}{c}{\textbf{Compress}} &
%   \multicolumn{1}{c}{\textbf{Csv}} &
%   \multicolumn{1}{c}{\textbf{Gson}} &
%   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Jackson}\\ \textbf{Core}\end{tabular}} &
%   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Jackson}\\ \textbf{Databind}\end{tabular}} &
%   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Jackson}\\ \textbf{Xml}\end{tabular}} &
%   \multicolumn{1}{c}{\textbf{Jsoup}} &
%   \multicolumn{1}{c}{\textbf{JxPath}} &
%   \multicolumn{1}{c}{\textbf{Lang}} &
%   \multicolumn{1}{c}{\textbf{Math}} &
%   \multicolumn{1}{c}{\textbf{Mockito}} &
%   \multicolumn{1}{c}{\textbf{Time}} &
%   \multicolumn{1}{c}{\textbf{Total}} \\ \midrule
% \# active defects   & 26 & 39 & 174 & 18 & 4 & 47 & 16 & 18 & 26 & 112 & 6 & 93 & 22 & 64  & 106 & 38 & 26 & 835 \\
% \# defects filtered          & 18 & 13 & 39  & 13 & 1 & 33 & 5  & 13 & 17 & 67  & 2 & 28 & 11 & 45  & 65  & 26 & 20 & 416 \\
% \# focal method & 30 & 20 & 48  & 24 & 3 & 42 & 7  & 30 & 48 & 115 & 2 & 41 & 21 & 149 & 124 & 43 & 36 & 783 \\ \bottomrule
% \end{tabular}
% }

% \end{table*}


\begin{table}[t]
\caption{Statistics of the bugs and focal methods in our study. Activate Defect (AD) refers to a defect that is reproducible. Filtered Defect (FD) refers to an active defect that has at least one focal method.}
\label{tab:defects4j}
\small
\begin{tabular}{l|rrr|l|rrr}
\toprule 
\textbf{Project} &
  \multicolumn{1}{l}{\textbf{\# AD}} &
  \multicolumn{1}{l}{\textbf{\# FD}} &
  \multicolumn{1}{l|}{\textbf{\# FM}} &
  \textbf{Project} &
  \multicolumn{1}{l}{\textbf{\# AD}} &
  \multicolumn{1}{l}{\textbf{\# FD}} &
  \multicolumn{1}{l}{\textbf{\# FM}} \\ 
\midrule
\textbf{Chart}        & 26  & 18 & 30 & \textbf{Jackson Databind} & 112 & 67 & 115 \\
\textbf{Cli}          & 39  & 13 & 20 & \textbf{Jsoup}            & 93  & 28 & 41  \\
\textbf{Closure}      & 174 & 39 & 48 & \textbf{JxPath}           & 22  & 11 & 21  \\
\textbf{Codec}        & 18  & 13 & 24 & \textbf{Lang}             & 64  & 45 & 149 \\
\textbf{Compress}     & 47  & 33 & 42 & \textbf{Math}             & 106 & 65 & 124 \\
\textbf{Csv}          & 16  & 5  & 7  & \textbf{Mockito}          & 38  & 26 & 43  \\
\textbf{Gson}         & 18  & 13 & 30 & \textbf{Time}             & 26  & 20 & 36  \\ 
\cline{5-8} 
\textbf{Jackson Core} & 26  & 17 & 48 &  \cellcolor[HTML]{EFEFEF}\textbf{\textit{Total}} &
  \cellcolor[HTML]{EFEFEF}\textbf{825} &
  \cellcolor[HTML]{EFEFEF}\textbf{413}	&
  \cellcolor[HTML]{EFEFEF}\textbf{778}
\\ \bottomrule
\end{tabular}
\end{table}

==> tables/humaneval_score.tex <==

\begin{table}[t]
\centering
\small
\caption{Pass@1 scores on HumanEval~\cite{humaneval} and EvalPlus~\cite{evalplus} benchmarks}
\label{tab:humaneval_score}
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Benchmark} &
  \multicolumn{2}{c}{{\ul CL}} &
  \multicolumn{2}{c}{{\ul DC}} &
  \multicolumn{1}{c}{{\ul PD}} &
  \multicolumn{1}{c}{\multirow{2}{*}{{\ul GPT-4}}} 
  \\
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{7B} &
  \multicolumn{1}{c}{13B} &
  \multicolumn{1}{c}{7B} &
  \multicolumn{1}{c}{33B} &
  \multicolumn{1}{c}{34B}  &
  \multicolumn{1}{c}{}
  \\ 
  \midrule
HumanEval & 34.8  & 42.7  & 78.6  & 79.3 & 73.8 & 88.4  \\
\midrule
EvalPlus & -  & -   & 70.1  & 72.6 & 67.1 &  76.8  \\
\bottomrule
\end{tabular}
\end{table}


==> tables/industry_result.tex <==
\begin{table}[t]
\caption{Evaluation results of DC-7B on two internal benchmarks.}
\label{tab:industry_results}
\centering
\begin{tabular}{@{}l|l|ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Group}} & \multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{3}{c}{\textbf{Metrics (\%)}}                                                                      \\
                       &                            & \multicolumn{1}{c}{$\bm{CSR}$} & \multicolumn{1}{c}{$\bm{Cov_{L}}$} & \multicolumn{1}{c}{$\bm{Cov_{B}}$} \\ 
                       \midrule
\multirow{3}{*}{w/o SFT} & BM  & 59.00 & 54.40 & 43.50 \\ 
                         & $BM_{easy}$ & 68.00 & 59.00 & 47.87 \\
                         & $BM_{hard}$ & 44.68  & 49.76  & 39.87  \\ \midrule
\multirow{3}{*}{SFT}     & BM  & 64.63 & 56.40 & 48.80 \\
                         & $BM_{easy}$ & 75.00 & 64.94 & 59.74 \\
                         & $BM_{hard}$ & 42.55 & 44.65 & 27.12  \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/rq1_compilable_details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Details About Coverage Scores Reached by Compilable Test Classes}
\label{tab:rq1_compilable}
\small
\begin{tabular}{@{}c|c|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\# Compilable UTs}} & \multicolumn{3}{c|}{\textbf{Line}}                & \multicolumn{3}{c}{\textbf{Branch}}             
\\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
       & 
       & \textbf{\# Covered} & \textbf{\# Total} & \textbf{$\bm{Cov}$(\%)}      & \textbf{\# Covered} & \textbf{\# Total} & \textbf{$\bm{Cov}$(\%)}       \\ \midrule
PD-34B & 1,738 & 2,608      & 4,249    & 61.38          & 1,599      & 3,434    & 46.56          \\
DC-33B & 1,882 & 2,818      & 4,494    & \textbf{62.71} & 1,781      & 3,588    & \textbf{49.64} \\
GPT-4                  & \textbf{1,951}                     & \textbf{3,502} & \textbf{6,101} & 57.40 & \textbf{2,119} & \textbf{4,721} & 44.88 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/rq1_focal_location.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\centering
\caption{Effective Comparison Between Different Location of Focal Method in Prompts}
\label{tab:rq1_focal_location}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
 &
  \multicolumn{3}{c|}{\textbf{CL-7B}} &
  \multicolumn{3}{c|}{\textbf{CL-13B}} &
  \multicolumn{3}{c|}{\textbf{PD-34B}} &
  \multicolumn{3}{c|}{\textbf{DC-7B}} &
  \multicolumn{3}{c}{\textbf{DC-33B}} \\
\multirow{-2}{*}{\textbf{Strategy}} &
  \textbf{$\bm{CSR}$} &
  \textbf{$\bm{Cov_{L}}$} &
  \textbf{$\bm{Cov_{B}}$} &
  \textbf{$\bm{CSR}$} &
  \textbf{$\bm{Cov_{L}}$} &
  \textbf{$\bm{Cov_{B}}$} &
  \textbf{$\bm{CSR}$} &
  \textbf{$\bm{Cov_{L}}$} &
  \textbf{$\bm{Cov_{B}}$} &
  \textbf{$\bm{CSR}$} &
  \textbf{$\bm{Cov_{L}}$} &
  \textbf{$\bm{Cov_{B}}$} &
  \textbf{$\bm{CSR}$} &
  \textbf{$\bm{Cov_{L}}$} &
  \textbf{$\bm{Cov_{B}}$} \\ \midrule
Begin &
  34.37 &
  16.21 &
  14.34 &
  38.95 &
  14.16 &
  12.18 &
  \textbf{56.06} &
  30.31 &
  24.14 &
  \textbf{50.27} &
  23.94 &
  17.20 &
  \textbf{50.54} &
  32.36 &
  26.76 \\
End &
  \textbf{37.95} &
  \textbf{17.50} &
  \textbf{14.62} &
  \textbf{50.64} &
  \textbf{21.66} &
  \textbf{18.01} &
  55.49 &
  \textbf{33.41} &
  \textbf{27.12} &
  49.22 &
  \textbf{29.02} &
  \textbf{23.77} &
  45.65 &
  \textbf{32.72} &
  \textbf{29.26} \\ \midrule
\multicolumn{1}{r|}{\textit{p-value}} &
  {\color{blue} 0.033} &
  {\color{blue} 3e-6} &
  {\color{blue} 1e-4} &
  {\color{blue} 9e-7} &
  {\color{blue} 1e-5} &
  {\color{blue} 1e-5} &
  {\color{red} 1.000} &
  {\color{blue} 0.011} &
  {\color{blue} 0.018} &
  {\color{red} 0.822} &
  {\color{blue} 3e-4} &
  {\color{blue} 3e-6} &
  {\color{blue} 5e-4} &
  {\color{red} 0.146} &
  {\color{blue} 0.035} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/rq1_num_tests.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The Number of Generated Unit Tests When Using Different Prompts.}
\label{tab:ablation_number_of_tests}
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Vaiants   & \multicolumn{1}{c}{CL-7B} & \multicolumn{1}{c}{CL-13B} & \multicolumn{1}{c}{PD-34B} & \multicolumn{1}{c}{DC-7B} & \multicolumn{1}{c}{DC-33B} \\ \midrule
All      & 3,378                     & 2,728                      & 2,651                      & 1,672                     & 3,238                      \\
w/o $FC_m$ & 4,177                     & 3,478                      & 3,783                      & 2,491                     & 4,233                      \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/rq2_order_compilation_rate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{Comparison of Compilation Success Rate Over Different Focal Method Location in Prompt.}
\label{tab:rq2_order_csr}
\begin{tabular}{@{}c|rrrrr|r@{}}
\toprule
\textbf{Location}              & \textbf{CL-7B}          & \textbf{CL-13B}         & \textbf{PD-34B}         & \textbf{DC-7B}          & \textbf{DC-33B}         
& \textbf{Avg.}
\\ \midrule
Origin Order & 40.31 &	50.64 &	55.49 &	49.22 &	45.65  &  \multicolumn{1}{c}{---}  \\
% Origin Order & \textcolor{blue}{$+3.58$}          &  \textcolor{blue}{$+11.69$}         &  \textcolor{red}{$-0.57$}       &  \textcolor{red}{$-1.05$}        &  \textcolor{red}{$-4.89$}         \\
At Begin       &
\textcolor{red}{$-3.58$} &	
\textcolor{red}{$-11.69$} &
\textcolor{blue}{$+0.57$} &
\textcolor{blue}{$+1.05$} &
\textcolor{blue}{$+4.89$} &
\textcolor{red}{$-1.75$} 
\\ 
% At Begin       & 34.37          & 38.95          & 56.06          & 50.27          & \textbf{50.54} \\
After  Constructor &
\textcolor{blue}{$+4.85$} & 	
\textcolor{blue}{$+3.43$} & 	
\textcolor{blue}{$+2.43$} & 	
\textcolor{blue}{$+1.56$} & 	
\textcolor{blue}{$+3.71$} & 	
\textcolor{blue}{$+3.20$} 


\\

% After  Constructor & \textbf{42.80} & 54.07          & \textbf{57.92} & 50.78          & 49.36          \\
After Fields &
\textcolor{red}{$-5.42$} &	
\textcolor{blue}{$+4.85$} &	
\textcolor{blue}{$+2.00$} &	
\textcolor{blue}{$+3.42$} &	
\textcolor{blue}{$+4.56$} &	
\textcolor{blue}{$+1.88$} 
\\



% After Fields       & 32.53          & \textbf{55.49} & 57.49          & \textbf{52.64} & 50.21          \\
 \bottomrule
\end{tabular}
\end{table}

==> tables/rq2_order_coverage.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\centering
\small
\caption{Comparison of Coverage Scores Over Different Focal Method Location in Prompt.}
\label{tab:rq2_order_cov}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\textbf{Location}} &
  \multicolumn{2}{c|}{\textbf{CL-7B}} &
  \multicolumn{2}{c|}{\textbf{CL-13B}} &
  \multicolumn{2}{c|}{\textbf{PD-34B}} &
  \multicolumn{2}{c|}{\textbf{DC-7B}} &
  \multicolumn{2}{c|}{\textbf{DC-33B}} 
  &
  \multicolumn{2}{c}{\textbf{Avg.}}\\ 
  % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
                   & \textbf{$\bm{Cov_{L}}$} & \textbf{$\bm{Cov_{B}}$} & \textbf{$\bm{Cov_{L}}$}  & \textbf{$\bm{Cov_{B}}$} & \textbf{$\bm{Cov_{L}}$}  & \textbf{$\bm{Cov_{B}}$} & \textbf{$\bm{Cov_{L}}$}  & \textbf{$\bm{Cov_{B}}$} & \textbf{$\bm{Cov_{L}}$}  & \textbf{$\bm{Cov_{B}}$}
                   & \textbf{$\bm{Cov_{L}}$}  & \textbf{$\bm{Cov_{B}}$}\\ \midrule




Origin Order &
18.76	& 
16.67	& 
21.66	& 
18.01	& 
33.41	& 
27.12	& 
29.02	& 
23.77	& 
32.72	& 
29.26 & \multicolumn{1}{c}{---} & \multicolumn{1}{c}{---} \\

  % \textcolor{blue}{$+1.29$} &
  % \textcolor{blue}{$+0.28$}&
  %  \textcolor{blue}{$+7.50$} &
  %  \textcolor{blue}{$+5.83$} &
  %  \textcolor{blue}{$+3.10$} &
  %  \textcolor{blue}{$+2.98$} &
  % \textcolor{blue}{$+5.08$} &
  % \textcolor{blue}{$+6.57$} &
  % \textcolor{blue}{$+0.36$} &
  % \textcolor{blue}{$+2.50$} \\ 
At Begin &
\textcolor{red}{$-1.29$} &
\textcolor{red}{$-0.28$} &
\textcolor{red}{$-7.50$} &
\textcolor{red}{$-5.83$} &
\textcolor{red}{$-3.10$} &
\textcolor{red}{$-2.98$} &
\textcolor{red}{$-5.08$} &
\textcolor{red}{$-6.57$} &
\textcolor{red}{$-0.36$} &
\textcolor{red}{$-2.50$} &
\textcolor{red}{$-2.89$} &
\textcolor{red}{$-3.63$} 
\\



% At Begin       & 16.21 & 14.34  & 14.16          & 12.18          & 30.31          & 24.14          & 23.94 & 17.20  & 32.36 & 26.76  \\
After  Constructor &
\textcolor{red}{$-0.31$} &
\textcolor{red}{$-1.60$} &
\textcolor{red}{$-0.33$} &
\textcolor{red}{$-0.37$} &
\textcolor{blue}{$+0.65$} &
\textcolor{blue}{$+0.95$} &
\textcolor{red}{$-3.10$} &
\textcolor{red}{$-1.71$} &
\textcolor{red}{$-2.04$} &
\textcolor{red}{$-3.97$} &
\textcolor{red}{$-0.85$} &	
\textcolor{red}{$-1.34$} 

\\
% After  Constructor & 17.19 & 13.02  & 21.33          & 17.64          & \textbf{34.06} & \textbf{28.07} & 25.92 & 22.06  & 30.68 & 25.29  \\
After Fields &
\textcolor{red}{$-6.07$} &
\textcolor{red}{$-6.36$} &
\textcolor{blue}{$+0.85$} &
\textcolor{blue}{$+0.92$} &
\textcolor{blue}{$+0.38$} &
\textcolor{blue}{$+1.12$} &
\textcolor{red}{$-3.96$} &
\textcolor{red}{$-3.63$} &
\textcolor{red}{$-0.87$} &
\textcolor{red}{$-1.67$} &
\textcolor{red}{$-1.61$} &
\textcolor{red}{$-1.92$} 
\\
% After Fields       & 11.43 & 8.26   & \textbf{22.51} & \textbf{18.93} & 33.79          & 28.24          & 25.06 & 20.14  & 31.85 & 27.59  \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/test_num.tex <==
\begin{table}[t]
\caption{Numbers of generated unit tests}
\begin{tabular}{l|ll|ll|l}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{CL}                           & \multicolumn{2}{c|}{DC}                           & \multicolumn{1}{c}{PD}  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{7B} & \multicolumn{1}{c|}{13B} & \multicolumn{1}{c}{7B} & \multicolumn{1}{c|}{33B} & \multicolumn{1}{c}{34B} \\
\midrule
no\_param\_constructor    & 20.78 & 20.44 & 8.311 & 14.60 & 9.942 \\
no\_class\_fields         & 21.69 & 22.27 & 8.686 & 14.86 & 10.04 \\
no\_param                 & 20.77 & 22.01 & 8.481 & 14.16 & 10.18 \\
no\_class\_other\_methods & 24.20 & 27.21 & 6.539 & 11.48 & 7.757 \\
no\_class\_constructor    & 20.85 & 21.81 & 7.874 & 13.44 & 10.30 \\
full                      & 20.75 & 21.95 & 8.688 & 14.29 & 9.862 \\
\bottomrule
\end{tabular}
\end{table}
